SGC: A semi-supervised pipeline for gene clustering using self-training approach in gene co-expression networks

A widely used approach for extracting information from gene expression data employ the construction of a gene co-expression network and the subsequent application of algorithms that discover network structure. In particular, a common goal is the computational discovery of gene clusters, commonly called modules. When applied on a novel gene expression dataset, the quality of the computed modules can be evaluated automatically, using Gene Ontology enrichment, a method that measures the frequencies of Gene Ontology terms in the computed modules and evaluates their statistical likelihood. In this work we propose SGC a novel pipeline for gene clustering based on relatively recent seminal work in the mathematics of spectral network theory. SGC consists of multiple novel steps that enable the computation of highly enriched modules in an unsupervised manner. But unlike all existing frameworks, it further incorporates a novel step that leverages Gene Ontology information in a semi-supervised clustering method that further improves the quality of the computed modules. Comparing with already well-known existing frameworks, we show that SGC results in higher enrichment in real data. In particular, in 12 real gene expression datasets, SGC outperforms in all except one.

==> TempTable.tex <==
\begin{minipage}{.60\textwidth}
  \centering
  \includegraphics[width= 1\linewidth]{SGC.pdf}
  \captionof{figure}{Overview of the SGC pipeline. The input is a gene expression matrix \( GE \) with \( m \) genes and \( n \) samples.}
  \label{fig:flowchart}
\end{minipage}%
\begin{minipage}{.38\textwidth}
 
 \begin{adjustbox}{width=.95\textwidth}
\begin{tabular}{||l c c c c c ||}
 \toprule
 \textbf{Data} & \textbf{Type} & \textbf{Organism} & \textbf{\#Samples} & \textbf{Unit} & \textbf{sft}  \\ 

\hline
\hline
GSE181225~\cite{GSE181225} &  RNA & Hs & 5 & RLE & 26 \\
\hline
GSE33779~\cite{GSE33779} & DNA & Dm & 90 & probes & 14 \\
\hline
GSE44903~\cite{GSE44903} & DNA & Rn & 142 & probes & 30 \\
\hline
GSE54456~\cite{GSE54456} & RNA & Hs & 174 & RPKM & 30 \\
\hline
GSE57148~\cite{GSE57148} & RNA & Hs & 189 & FPKM & 14 \\
\hline
GSE60571~\cite{GSE60571} & RNA & Dm & 235 & FPKM & 9 \\
\hline
GSE107559~\cite{GSE107559} & RNA & Hs & 270 & FPKM & 3 \\
\hline
GSE28435~\cite{GSE28435} & DNA & Rn & 335 & probes & 22 \\
\hline
GSE104687~\cite{GSE104687} & RNA & Hs & 377 & FPKM & 18 \\
\hline
GSE150961~\cite{GSE150961} & RNA & Hs & 418 & TMM & 5 \\
\hline
GSE115828~\cite{GSE115828} & RNA & Hs & 453 & CPM & 12 \\
\hline
GSE38705~\cite{GSE38705} & DNA & Mm & 511 & probes & 1 \\
\hline
\hline
\bottomrule
\end{tabular}
\end{adjustbox}

\qquad

\begin{adjustbox}{width=.95\textwidth}
\begin{tabular}{||l || c c || c c || c c || c c || c c ||}
  \toprule
  & \multicolumn{2}{|c|}{WGCNA} & \multicolumn{2}{|c|}{CoExpNets} & \multicolumn{2}{|c|}{CEMiTool} & \multicolumn{2}{|c|}{pSGC} & \multicolumn{2}{|c|}{SGC} \\
  
\hline
\hline
GSE181225~\cite{GSE181225} & 48 & 7462 & 75 & 9027 & 32 & 6252 & 2 & 2598 & 2 & 2598 \\
\hline
GSE33779~\cite{GSE33779} & 22 & 5631 & 19 & 6213  & 17 & 5299 & 10 & 4144 & 7 & 3821 \\
\hline
GSE44903~\cite{GSE44903} & 18 & 3298 & 27 & 4705 & 14 & 3303 & 4 & 987 & 4 & 1059 \\
\hline
GSE54456~\cite{GSE54456} & 31 & 9386 & 46 & 14473 & 22 & 11056 & 3 & 6004 & 3 & 600 \\
\hline
GSE57148~\cite{GSE57148} & 45 & 13296 & 36 & 14110 & 33 & 12027 & 9 & 2833 & 5 & 2383 \\
\hline
GSE60571~\cite{GSE60571} & 21 & 7107 & 19 & 8622 & 16 & 5564 & 2 & 2969 & 2 & 2971 \\
\hline
GSE107559~\cite{GSE107559} & 26 & 10915 & 20 & 12499  & 80 & 15952 & 14 & 5257 & 12 & 4913 \\
\hline
GSE28435~\cite{GSE28435} & 51 & 7331 & 47 & 7769 & 31 & 6566 & 2 & 2052 & 2 & 2053  \\
\hline
GSE104687~\cite{GSE104687} & 31 & 10339 & 28 & 1193 & 23 & 11369 & 2 & 6426 & 2 & 6426  \\
\hline
GSE150961~\cite{GSE150961} & 9 & 3619 & 18 & 606 & 17 & 4856 & 2 & 2111 & 2 & 2111  \\
\hline
GSE115828~\cite{GSE115828} & 51 & 12611 & 10 & 7693 & 10 & 5231 & 3 & 1934 &  3 & 1926 \\
\hline
GSE38705~\cite{GSE38705} & 8 & 3320  & 12 & 4123 & 7 & 3308 & 6 & 2824 & 4 & 2610 \\

\hline
\hline

\bottomrule

 \end{tabular}
\end{adjustbox} 
\end{minipage}

 
\begin{table}
    \caption{Semi-labeling summary. For each data, the percentage of the remarkable genes and the percentage of unremarkable genes that their label have changed after semi-supervised is given.}
    \label{tab:semilabelingSummary}
    \begin{adjustbox}{width=\textwidth}
        \begin{tabular}{||l c c  || l c c  || l c c  ||} 
         \hline
         Data && Data & \% Unremarkable Genes & \% Changed Label & Data & \% Unremarkable Genes & \% Changed Label \\  
         \hline\hline
         GSE181225 & 1\% & 0\% & GSE33779 & 56\% & 47.1\% & GSE44903 & 29\% & 5\%  \\ 
         \hline
         GSE54456 & 1\% & 1\% & GSE57148 & 46\% & 24\% & GSE60571 & 21\% & 2\%  \\ 
         \hline
         GSE107559 & 6\% & 48.4\% & GSE28435 & 12\% & 0\% & GSE104687 & 0\% & 0\%  \\ 
         \hline
         GSE150961 & 9\% & 0\% & GSE115828 & 33\% & 0\% & GSE38705 & 39\% & 62\%  \\ 
         \hline
         \hline
        \end{tabular}
    \end{adjustbox}
\end{table}


==> other.tex <==

\begin{comment}
\par \textbf{iv. Odds Ratios for GO terms.} \autoref{fig:OddsRatioPlot} shows the {\em odds ratio} value associated to each GO term. The {\em odds ratio} is defined as the proportion of a GO term genes within a module to the proportion of this GO term genes in the dataset. More precisely, it evaluates the strength of the GO term within a module~\cite{MOET}. As usual, the higher the {\em odds ratio}, the more stronger the enrichment. Here, the odds values are discretized into four bins; 0, less equal to 1 (~\( \le 1\)), greater than 1~(~\( \geq 1 \)), and infinity \( (+Inf) \). The percentage of the GO terms that their corresponding {\em odds ratio} fall in each bin was calculated for each pipeline on the \( 12 \) data individually. The zero {\em odds ratio} occurs if none of the GO term genes in the data fall in the module, however, the {\em p-value} of the term is significant. All pipelines have very similar percentages of genes with zero {\em odds ratio} except GSE60571, and GSE115828 in which pSGC and SGC have a smaller number of GO terms for this bin; this is reversed for GSE181225.
The infinity {\em odds ratio} (orange stack) occurs if all the genes associated to a GO term in the dataset fall in the same module. This mostly occurs mostly on GSE181225 in the case of WGCNA, CoExpNets, and CEMiTool. On the other hand psGC and SGC have, more gnes with an infinite odds ratio for GSE54456, GSE57148, GSE104687, GSE107559 for pSGC, SGC. Interestingly, with the exception of GSE5714 these are the datasets where SGC is {\em dominant} to the other frameworks, in the sense explained above. 

Looking at the red and green stacks in~\autoref{fig:OddsRatioPlot} we see that SGC tends to find {\em less} genes with an odds ratio higher than 1 in their corresponding module. This is consistent with the overall behavior of SGC: As an example, suppose two equal-size groups of genes $A$ and $B$ both associated with a GO term are placed into different modules. Then, the corresponding GO term will be reported for both modules, but their odds ratios will be modest; possibly higher than 1, but not much. On the other hand, if most genes of $B$ go into the same module with $A$, that can generate a GO term with an odds ratio of less than $1$, and one with a very high odds ratio. In summary then, SGC appears to be able to highlight fewer GO terms but with very high odds ratio. In principle that means that SGC can highlight the significance of GO terms that are missed by the other three frameworks. 
\end{comment}


==> steps.tex <==
1/Gene Semi-labeling
2/ Semi-supervised Classification
3/ first, second, gap, f, s, g => relative gap, second-order gap, additive order, rg, sg, ag


